Graph Clustering Bandits for Recommendation

We investigate an efficient context-dependent clustering technique for recommender systems based on exploration-exploitation strategies through multi-armed bandits over multiple users. Our algorithm dynamically groups users based on their observed behavioral similarity during a sequence of logged activities. In doing so, the algorithm reacts to the currently served user by shaping clusters around him/her but, at the same time, it explores the generation of clusters over users which are not currently engaged. We motivate the effectiveness of this clustering policy, and provide an extensive empirical analysis on real-world datasets, showing scalability and improved prediction performance over state-of-the-art methods for sequential clustering of users in multi-armed bandit scenarios.

==> abstract_intro.tex <==


\begin{abstract} 
%updated the abs to best fit the space and better considered description by shuai
We introduce a novel algorithmic approach to content-based recommendation system
% in interacting user scenarios (e.g., a social network) 
with the adaptive clustering of exploration-exploitation (``bandit") tradeoff strategies. 
We provide a sharp regret analysis of this algorithm in a standard stochastic 
noise setting, demonstrate its scalability properties, and 
prove its effectiveness on both a number of artificial and real-world datasets.
Our experiments show a significant increase in prediction performance
over state-of-the-art methods for bandit problems. 
%
\iffalse
********************
{\bf GZ: tentative}
Contextual bandit problems formalize the exploration-exploitation dilemma arising in several industrial applications, such as online advertisement and, more generally, recommendation systems.
In some of these applications such webpages personalization, the algorithm should learn a model for each user of the website starting with little or no information.
In practice, it is often the case that a user is not completely different from each other, and in general, it is often possible to find a small set of models those represents the preferences of all the users creating in this way a cluster of users for each model.

Unfortunately, the learner does not have any previous knowledge on the similarity among the users, on the candidate models or on the number of models those are necessary to represent all the users.
The only viable way for the learner to exploit this similarity is to learn a clusterization of the users while it learns the models, \textit{betting} on the fact that the number of distinct models will be much smaller than the total number of users.

In this paper we present an algorithm for learning similarity and sharing feedback among multiple linear bandit problems, while obtaining a regret bound that depends on the real number of clusters instead of on the number of users. 
The last part of the paper is dedicated to compare our algorithm with the state of the art algorithms for linear bandits.
*********************
\fi
\end{abstract} 

\vspace{-0.25in}



\section{Introduction}
%
\vspace{-0.05in}
Presenting personalized content to users is nowdays a crucial functionality for many online 
recommendation services. Due to the ever-changing set of available options, these services 
have to exhibit strong adaptation capabilities when trying to match 
%as much as possible the 
users' preferences. 
%In essence, 
Coarsely speaking, the underlying systems repeatedly learn a mapping between available content 
and users, the mapping being based on {\em context} information (that is, sets of features) which is 
typically extracted from both users and contents. 
The need to focus on content that raises the users' interest, 
combined with the need of exploring new content so as to globally improve users' experience, 
generates a well-known exploration-exploitation dilemma, which is commonly formalized as 
a multi-armed bandit problem~(e.g., \cite{lr85,ACF01,audibert:hal-00711069,CaronKLB12}). 
In particular, the contextual bandit methods~(e.g., \cite{Aue02,lz07,li2010contextual,chu2011contextual,
bogers2010movie,abbasi2011improved,cg11,ko11}, and references therein) 
have rapidly become a reference algorithmic technique for implementing adaptive recommender systems.

\vspace{-0.05in}
% new challenge: users are increasing in number, and interact
Within the above scenarios, the widespread adoption of online social networks, where users are 
engaged in technology-mediated social interactions (making product endorsement and word-of-mouth 
advertising a common practice), raises further challenges and opportunities to content recommendation 
systems: On one hand, because of the mutual influence among friends, acquaintances, business partners, 
etc., users having strong ties are more likely to exhibit similar interests, and therefore similar 
behavior. On the other hand, the nature and scale of such interactions calls for adaptive
algorithmic solutions which are also computationally affordable.

\vspace{-0.05in}
% two approaches: explicit networks and implicit networks
Incorporating social components into bandit algorithms can lead to a dramatic increase in the quality 
of recommendations. For instance, we may want to serve content to a group of users by taking advantage of 
an underlying network of social relationships among them. These social relationships can either be 
explicitly encoded in a graph, where adjacent nodes/users are deemed similar to one another, or implicitly
contained in the data, and given as the outcome of an inference process that recognizes similarities 
across users based on their past behavior. 
Examples of the first approach are the recent works~\cite{bes13,dkmc13,cgz13}, where
a social network structure over the users is assumed to be given that reflects actual interest similarities
among users -- see also \cite{cb13, valko2014spectral} for recent usage of social information to tackle the so-called 
``cold-start" problem. Examples of the second approach are the more traditional 
collaborative-filtering (e.g.,~\cite{skr99}), content-based filtering, and hybrid approaches (e.g.~\cite{b05}).
Both approaches have important drawbacks hindering their practical deployment. One obvious drawback
of the ``explicit network" approach is that the social network information may be misleading
%(e.g., ``is it really true that if we are friends in Facebook then we like the same books ?") 
(see, e.g., the experimental evidence reported by~\cite{dkmc13}), or simply unavailable. 
Moreover, even in the case when this information is indeed available and useful, 
the algorithmic strategies to implement the needed feedback sharing mechanisms might lead to severe 
scaling issues~\cite{cgz13}, especially when the number of targeted users is large.
A standard drawback of the ``implicit network" approach of traditional recommender systems 
is that in many practically relevant scenarios (e.g., web-based), content universe and popularity often 
undergo dramatic changes, making these approaches difficult to apply. 

\vspace{-0.05in}
In such settings, most notably in the relevant case 
when the involved users are many, it is often possible to identify 
a few subgroups or communities within which users share similar interests~\cite{rlkr06,bwdh12},
%~\cite{xlyxzyc05,rlkr06,bwdh12}, 
thereby greatly facilitating 
the targeting of users by means of {\em group} recommendations. Hence the system need not learn 
a different model for each user of the service, but just a single model for each group. 

\vspace{-0.05in}
In this paper, we initiate\footnote
{
The only paper we are aware of which has similar goals as ours is~\cite{bkm12}, though that 
paper apparently works under more restrictive assumptions.
} 
a theoretical and experimental investigation of adaptive clustering algorithms
for linear (contextual) bandits under the assumption that we have to serve content to a set of $n$ users 
organized into $m << n$ groups (or {\em clusters}) such that users within each group tend to provide
similar feedback to content recommendations. We give a $O(\sqrt{T})$ regret analysis holding in a standard
stochastically linear setting for payoffs where, importantly, the hidden constants in the big-oh 
depend on $m$, rather than $n$, as well as on the geometry of the user models within the different 
clusters.
%
The main idea of our algorithm is to use confidence balls of the users' models to both estimate user similarity, 
and to share feedback across (deemed similar) users. The algorithm adaptively interpolates between
the case when we have a single instance of a contextual bandit algorithm making the same predictions for all 
users and the case when we have $n$-many instances providing fully personalized recommendations.
We show that our algorithm can be implemented efficiently (the large $n$ scenario being of special concern here) 
by means of off-the-shelf data-structures relying on random graphs. Finally, we test our algorithm 
on medium-size synthetic and real-world datasets, often reporting a significant increase in prediction performance
over known state-of-the-art methods for bandit problems. 




\iffalse
In practice, it is often the case that the system does not need to learn a different model for each single user of the service, but it can just learn a model for each cluster of users with similar taste. 
This problem has somehow already been addressed in previous papers, assuming that side information from a social network among the users was provided to the algorithm (i.e., see \cite{}). 
Unfortunately, it is not always the case: in some cases there is not information available about the users except their current behavior, and even when the side information is available it may not provide good similarity information. %This will also address the problem of learning personalized models when the users interact with the service very few times.
Learning the similarity among the users while learning their preferences model is far from trivial.\\
In this work, we provide an algorithm for contextual bandits able to learn and leverage the similarity among the users. 

The main idea is to use the confidence balls of the users' models to estimate the similarity among the users and in this way allow the algorithm to share feedback among similar users.
This mechanism is implemented running a single contextual bandit algorithm for each cluster of users, using all the feedback obtained for all the predictions made for the users in the cluster.
Roughly speaking, the algorithm interpolates between the case where there is only one instance of a contextual bandits making predictions for all the users and the case where there is a single instance of a contextual bandit algorithm for each user.\\
In the last part of the paper, we present a comparison between the new algorithm and the state of the art linear bandit algorithms in a completely controlled environment.
Oftentimes our algorithm outperforms its competitors and it is never worse than the best among them.
\fi





==> alg.tex <==



%\vspace{-0.1in}
\section{The Algorithm}\label{s:alg}
%
%\vspace{-0.05in}
Our algorithm, called Graph Cluster of Bandits (GCLUB, see Figure \ref{alg:gclub}), is a variant of the Cluster of Bandits (CLUB) algorithm originally introduced in \cite{icml14}. We first recall how CLUB works, point out its weakness, and then describe the changes that lead to the GCLUB algorithm.

The CLUB algorithm maintains over time a partition of the set of users $\scU$ in the form of {\em connected components} of an undirected graph $G_t =(\scU,E_t)$ whose nodes are the users, and whose edges $E_t$ encode our current belief about user similarity. CLUB starts off from a randomly sparsified version of the complete graph (having $\scO(n\log n)$ edges instead of $\scO(n^2)$), and then progressively deletes edges based on the feedback provided by the current user $i_t$. Specifically, each node $i$ of this graph hosts a linear function $\bw_{i,t}\,: \bx \rightarrow \bw_{i,t}^\top\bx$ which is meant to estimate the payoff user $i$ would provide had item $\bx$ been recommended to him/her. The hope is that this estimates gets better and better over time. When the current user is $i_t$, it is only vector $\bw_{i_t,t}$ that is updated based on $i_t$'s payoff signal, similar to a standard linear bandit algorithm (e.g.,~\cite{Aue02,chu2011contextual,abbasi2011improved,cgz13}) operating on the context vectors contained in $C_{i_t}$. Every user $i \in \scU$ hosts such a linear bandit algorithm. The actual recommendation issued to $i_t$ within $C_{i_t}$ is computed as follows. First, the connected component (or cluster) that $i_t$ belongs to is singled out (this is denoted by $\hj_t$ in Figure \ref{alg:gclub}). Then, a suitable aggregate prediction vector (denoted by $\bbw_{\hj_t,t-1}$ in Figure \ref{alg:gclub}) is constructed which collects information from all uses in that connected component. The vector so computed is engaged in a standard upper confidence-based exploration-exploitation tradeff to select the item ${\bar \bx_t} \in C_{i_t}$ to recommend to user $i_t$. 

Once $i_t$'s payoff $a_t$ is received, $\bw_{i_t,t-1}$ gets updated to $\bw_{i_t,t}$ (through $a_t$ and ${\bar \bx_t}$). In turn, this may change the current cluster structure, for if $i_t$ was formerly connected to, say, node $\ell$ and, as a consequence of the update $\bw_{i_t,t-1} \rightarrow \bw_{i_t,t}$, vector $\bw_{i_t,t}$ is no longer close to $\bw_{\ell,t-1}$, then this is taken as a good indication that $i_t$ and $\ell$ cannot belong to the same cluster, so that edge $(i_t,\ell)$ gets deleted, and new clusters over users are possibly obtained.

The main weakness of CLUB in shaping clusters is that when responding to the current user feedback, the algorithm operates only {\em locally} (i.e., in the neigborhood of $i_t$). While advantageous from a computational standpoint, in the long run this has the severe drawback of overfocusing on the (typically few) very active users; the algorithm is not responsive enough to those users on which not enough information has been gathered, either because they are not so active (typically, the majority of them) or because they are simply newly registered users. In other words, in order to make better recommendations it's worthy to discover and capture the ``niches'' of user preferences as well. 

Since uneven activity levels among users is a standard pattern when users are many (and this is the case with our data, too --- see Section \ref{s:exp}), GCLUB complements CLUB with a kind of stochastic exploration at the level of cluster shaping. In every round $t$, GCLUB deletes edges in one of two ways: with independent high probability $1-r > 1/2$, GCLUB operates on component $\hj_t$ as in CLUB, while with low probability $r$ the algorithm picks a connected component uniformly at random among the available ones at time $t$, and splits this component into {\em two} subcomponents by invoking a fast graph clustering algorithm (thereby generating  one more cluster). This stochastic choice is only made during an initial stage of learning (when $t \leq T/10$ in GCLUB's pseudocode), which we may think of as a {\em cold start} regime for most of the users.
The graph clustering algorithm we used in our experiments was implemented through the {\em Graclus} software package from the authors of \cite{pami07,sigkdd05}. Because we are running it over a single connected component of an initially sparsified graph, this tool turned out to be quite fast in our experimentation. 

The rationale behind GCLUB is to add an extra layer of exploration-vs-exploitation tradeoff, which operates at the level of clusters.
% the algorithm decides to deal with. 
At this level, exploration corresponds to picking a cluster at random among the available ones, while exploitation corresponds to working on the cluster the current user belongs to. In the absence of enough information about the current user and his/her neighborhood, exploring other clusters is intuitively beneficial. We will see in the next section that this is indeed the case.
%
\begin{figure}[t!]
\begin{center}
\begin{algorithmic}
\small
%\vspace{-1.4in}
\STATE \textbf{Input}: Exploration parameter $\alpha > 0$; 
%edge deletion parameter $\alpha_2 > 0$; 
cluster exploration probability $r < 1/2$.
\STATE \textbf{Init}:
%\vspace{-0.1in}
\begin{itemize}
\item $\bb_{i,0} = \bzero \in \R^d$ and $M_{i,0} = I \in \R^{d\times d}$,\ \ $i = 1, \ldots n$;
%\vspace{-0.1in}
\item Clusters ${\hat U_{1,1}} = \scU$, number of clusters $m_1 = 1$;
%\vspace{-0.1in}
\item Graph $G_1 = (\scU,E_1)$, $G_1$ has $\scO(n\log n)$ edges and is connected.
\end{itemize}
%\vspace{-0.1in}
\FOR{$t =1,2,\dots,T$}
\STATE Receive $i_t \in \scU$;
%\IF {$t \leq T \times 20\%$}
%	\STATE With probability $\rho$ conduct the cold start training boosted exploration: pick one cluster uniformly at random, execute one fast graph clustering procedure and delete edges correspondingly by ending up with one more clusters;%the fast graph (mincut-like) clustering tool: graclus
	%\STATE With high probability $\rho$ locate the cluster that current served user $i_t$ belongs to, within that cluster find the $i_t$'s neighborhood set that made up of directed connected user, delete the edges among them
%\ENDIF 
%\COMMENT{This is a comment statement}
\STATE Set $\bw_{i,t-1} = M_{i,t-1}^{-1}\bb_{i,t-1}$, \quad $i = 1, \ldots, n$;
\STATE Get item set
       $
       C_{i_t} = \{\bx_{t,1},\ldots,\bx_{t,c_t}\};
       $
\STATE Determine $\hj_t \in \{1, \ldots, m_t\}$ such that $i_t \in {\hat U_{\hj_t,t}}$, and set
%\vspace{-0.1in}
\begin{align*}
   \bM_{{\hj_t},t-1}  &= I+\sum_{i \in {\hat U_{\hj_t,t}}} (M_{i,t-1}-I),\\
   \bbb_{{\hj_t},t-1} &= \sum_{i \in {\hat U_{\hj_t,t}}} \bb_{i,t-1},\\
   \bbw_{{\hj_t},t-1} &= \bM_{{\hj_t},t-1}^{-1}\bbb_{{\hj_t},t-1}~;
\end{align*}
%\vspace{-0.25in}
\STATE \[
       {\mbox{Set\ \ }}
        k_t = \argmax_{k = 1, \ldots, c_t} \left({\bbw_{\hj_t,t-1}}^\top\bx_{t,k}  + \CB_{\hj_t,t-1}(\bx_{t,k})\right),
       \]
%\vspace{-0.15in}
       \begin{align*}
       {\mbox{where\ \ }}
       \CB_{{\hj_t},t-1}(\bx) &= \alpha\,\sqrt{\bx^\top \bM_{{\hj_t},t-1}^{-1} \bx\,\log(t+1)}\,.%\ j = 1, \ldots, m_t~,
      % \bM_{j,t-1} &= I+\sum_{i \in {\hat U_{j,t}}} (M_{i,t-1}-I)\,,\quad j = 1, \ldots, m_t~.
       \end{align*}
%\vspace{-0.1in}
\STATE Observe payoff $a_t \in [-1,1]$;
\STATE Let ${\bar \bx_t} = \bx_{t,k_t}$;
\STATE Update weights:
       \begin{itemize}
 %      \vspace{-0.1in}
       \item $M_{i_t,t} = M_{i_t,t-1} + {\bar \bx_{t}}{\bar \bx_{t}}^\top$,
 %      \vspace{-0.1in}
       \item $\bb_{i_t,t} = \bb_{i_t,t-1} + a_t {\bar \bx_t}$,
 %      \vspace{-0.1in}
       \item Set $M_{i,t} =  M_{i,t-1},\ \bb_{i,t} = \bb_{i,t-1}$ for all $i \neq i_t$~;
       \end{itemize}
\STATE Update clusters:
\begin{itemize}
%\vspace{-0.06in}
\item Flip independent coin $X_t \in \{0,1\}$ with $\Pr(X_t = 1) = r$.
       \begin{itemize}
 %      \vspace{-0.12in}
       \item If $X_t = 0$ then delete from $E_t$ all $(i_t,\ell)$ such that
       \[
             ||\bw_{i_t,t-1} - \bw_{\ell,t-1}|| > \sCB_{i_t,t-1} + \sCB_{\ell,t-1}~,
       \]
%      where
  %     \vspace{-0.3in}
       \begin{align*}
        \sCB_{i,t-1} &= \alpha\,\sqrt{\frac{1+\log(1+T_{i,t-1})}{1+T_{i,t-1}}},\\
        T_{i,t-1}    &= |\{s \leq t-1\,:\, i_s = i \}|,\qquad i \in \scU;
       \end{align*}
   %    \vspace{-0.28in}
       \item If $X_t = 1$ and $t \leq T/10$ then pick at random index $j \in \{1, \ldots, m_t\}$, $j \neq \hj_t$, and split $\hat U_{j,t}$ into two subclusters $\hat U_{j,t,1}$ and $\hat U_{j,t,2}$ by means of a standard graph clustering procedure. Delete all edges between $\hat U_{j,t,1}$ and $\hat U_{j,t,2}$.
\end{itemize}
%\vspace{-0.15in}
\item Let $E_{t+1}$ be the resulting set of edges, set $G_{t+1} = (\scU,E_{t+1})$,
        and compute associated clusters
        $\hat U_{1,t+1}, \hat U_{2,t+1}, \ldots, \hat U_{m_{t+1},t+1}$~.
\end{itemize}
\ENDFOR
\end{algorithmic}
%\vspace{-0.1in}
\caption{\label{alg:gclub}
Pseudocode of the GCLUB algorithm.
%\vspace{-0.45in}
}
\end{center}
%\vspace{-0.25in}
\end{figure}
%
% 

\iffalse
***************************************************************
At each time $t=1,2,\dots$, the algorithm receives the index $i_t$ of the user to serve, and the
associated context vectors $\bx_{t,1}, \ldots, \bx_{t,c_t}$
(the set $C_{i_t}$), and must select one among them. In doing so, the algorithm first determines
which cluster node $i_t$ belongs to, among those available at time $t$,
and then builds the aggregate weight vector
$\bbw_{\hj_t,t-1}$ by taking prior ${\bar \bx_s}$, $s < t$


belonging to the users in cluster and


computing the least squares approximation as if all nodes
$i \in \hat V_{\hj_t,t}$ have been collapsed into one.

The quantity
$\CB_{\hj_t,t-1}(\bx)$ is a version of the upper confidence bound in the approximation of
$\bbw_{\hj_t,t-1}$ to a suitable combination
of vectors $\bu_i$, $i \in {\hat V_{\hj_t,t}}$ -- see Lemma \ref{l:comboapprox} in the supplementary
material.

Once this selection is done and the associated payoff $a_t$ is observed, the algorithm uses the selected vector
${\bar \bx_t}$ for updating $M_{i_t,t-1}$ to $M_{i_t,t}$ via a rank-one adjustment,
and for turning vector $\bb_{i_t,t-1}$ to $\bb_{i_t,t}$
via an additive update whose learning rate is precisely $a_t$.
Notice that the update is only performed at node $i_t$, since for all other $i \neq i_t$ we have
$\bw_{i,t} = \bw_{i,t-1}$. However, this update at $i_t$ will also implicitly update the
aggregate weight vector $\bbw_{\hj_{t+1},t}$ associated with cluster ${\hat V_{\hj_{t+1},t+1}}$ that node $i_t$
will happen to belong to in the next round.
% not at node $\hs_t$.

Finally, the cluster structure is possibly modified:
CLUB compares, for any existing edge $(i_t,\ell) \in E_{t}$, the distance
\(
||\bw_{i_t,t-1}- \bw_{\ell,t-1}||
\)
between
%the projected
vectors $\bw_{i_t,t-1}$ and $\bw_{\ell,t-1}$
to the quantity
\(
\sCB_{i_t,t-1} + \sCB_{\ell,t-1}~.
\)
If the above distance is significantly large (and $\bw_{i_t,t-1}$ and $\bw_{\ell,t-1}$ are good approximations to
the respective underlying vectors $\bu_{i_t}$ and $\bu_{\ell}$),
%
% then we expect that both $\sCB_{i_t,t}$ and
% $\sCB_{j,t}$ are small, making
%
then this is a good indication that
$\bu_{i_t} \neq \bu_{\ell}$ (i.e., that node $i_t$ and node $\ell$ cannot belong to the same true cluster), so that
edge $(i_t,\ell)$ gets deleted.
The new graph $G_{t+1}$, and the induced partitioning clusters $\hat V_{1,t+1}, \hat V_{2,t+1}, \ldots, \hat V_{m_{t+1},t+1}$,
%and associated representatives $\hs_{1,t+1}, \hs_{2,t+1}, \ldots, \hs_{m_{t+1},t+1}$
are then computed, and a new round begins.
****************************************************
\fi



==> conclusions.tex <==

\section{conclusions}

one may wonder: 1) why not invoking graclus over the whole graph every round: this would be too computationally expensive; 
2) why not use your boosted strategy all the way to the end (rather than only in the training stage).



==> experiments.tex <==

%\vspace{-0.18in}
\section{Experiments}\label{s:exp}
%
In this section, we briefly describe the setting and the outcome of our experimental investigation.

\subsection{Datasets}
We tested our algorithm on four freely available real-world benchmark datasets against standard bandit baselines for multiple users.

\textbf{LastFM, Delicious, and Yahoo datasets.}
For the sake of fair comparison, we carefully followed and implemented the experimental setup as described in~\cite{icml14} on these datasets, we refer the reader to that paper for details. The Yahoo dataset is the one called `` Yahoo 18k" therein.

\textbf{MovieLens dataset.} This is the freely available\footnote
{
http://grouplens.org/datasets/movielens~.
}
benchmark dataset MovieLens 100k.
In this dataset, there are $100,000$ ratings from $n = 943$ users on $1682$ movies, where each user has rated at least $20$ movies. Each movie comes with a number of features, like id, movie title, release date, video release date, and genres. After some data cleaning,
%by filtering out the outlier records whose some fields are missing or mismatch as the outlier. Second,
we extracted numerical features through a standard tf-idf procedure.
%term weighting (term-frequency times inverse document-frequency)
%where those fields' type are string.
We then applied PCA %(principal component analysis)
to the resulting feature vectors so as to retain at least $95\%$ of the original variance, giving rise to item vectors $\bx_{t,k}$ of dimension $d=19$. Finally, we normalized all features so as to have zero (empirical) mean and unit (empirical) variance. As for payoffs, we generated binary payoffs, by mapping any nonzero rating to payoff 1, and the zero rating to payoff 0. Moreover, for each timestamp in the dataset referring to user $i_t$, we generated random item sets $C_{i_t}$ of size $c_t = 25$ for all $t$ by putting into $C_{i_t}$ an item for which $i_t$ provided a payoff of 1, and then picking the remaining 24 vectors at random from the available movies up to that timestamp. Hence, each set $C_{i_t}$ is likely to contain only one (or very few) movie(s) with payoff 1, out of 25. The total number of rounds was $T = 100,000$. We took the first $10K$ rounds for parameter tuning, and the rest for testing.

In Figure \ref{fig:activity_level}, we report the activity level of the users on the Yahoo and the MovieLens datasets. As evinced by these plots,\footnote
{
%Due to space limitations, //refined by Shuai
Without loss of generality, we take these two datasets to provide statistics, but similar shapes of the plots can be established for the other two datasets.
}
such levels are quite diverse among users, and the emerging pattern is the same across these datasets: there are few very engaged users and a long tail of (almost) unengaged ones.
%
%
\begin{figure}[t!]
\begin{picture}(22,25)(22,25)
\begin{tabular}{l@{\hspace{-1.7pc}}l}
\includegraphics[width=0.29\textwidth]{plots/yahooDist2.pdf}
%\includegraphics[scale=0.23]{plots/yahooDist2.pdf}
& \includegraphics[width=0.29\textwidth]{plots/movielensDist.pdf}
%& \includegraphics[scale=0.23]{plots/movielensDist.pdf}
\end{tabular}
\end{picture}
\vspace{0.9in}
\caption{\label{fig:activity_level} User activity levels on the Yahoo (left) and the MovieLens (right) datasets. Users are sorted in decreasing order according to the number of times they provide feedback to the learning system. For the sake of better visibility, on the Yahoo dataset we truncated to the 2K most active users (out of 18K).
}
%\vspace{-0.10in}
\end{figure}
%

% in the criteria that it maintains the original variance by $\%95$ fraction.
% Fourth, we normalize all features by subtracting mean and divided by stand deviation respectively. Fiveth, we binarize each user's rating where non-zero rating as reward $1$ otherwise $0$, that is, for each timestamp's recommendation list there is one and only one item with payoff $1$, the rest positions for recommending is composed of other movie id by uniformly pick at random based on the movies seen up to  that timestamp by the system. And then, we drop the first $25$ records in database as the initial pool for recommendation list's construction.

%Finally we use the hash table to build the mapping relationship, then re-order the user id and movie id correspondingly. After this data curation process this dataset ends up with number of records $=99,976$, feature dimension $=19$, recommendation list's length $=25$.

\subsection{Algorithms}
We compared GCLUB to three representative competitors: LinUCB-ONE, LinUCB-IND, and CLUB.
LinUCB-ONE and LinUCB-IND are members of the LinUCB family of algorithms~\cite{Aue02,chu2011contextual,abbasi2011improved,cgz13} and are, in some sense, extreme solutions: LinUCB-ONE allocates a single instance of LinUCB across all users (thereby making the same prediction for all users -- which would be effective in a {\em few-hits} scenario), while LinUCB-IND (``LinUCB INDependent") allocates an independent instance of LinUCB to each user, so as to provide personalized recommendations (which is likely to be effective in the presence of {\em many niches}). CLUB is the online clustering technique from \cite{icml14}. On the Yahoo dataset, we run the featureless version of the LinUCB-like algorithm in~\cite{cgz13}, i.e., a version of the UCB1 algorithm of~\cite{ACF01}. The corresponding ONE and IND versions are denoted by UCB-ONE and UCB-IND, respectively. Finally, all algorithms have also been compared to the trivial baseline (denoted here as RAN) that selects the item within $C_{i_t}$ fully at RANdom.

We tuned the parameters of the algorithms in the training set with a standard grid search as in \cite{icml14}, and used the test set to evaluate predictive performance.
%The cluster exploration probability $r$ in GCLUB was set to 0.3
The training set was about 10\% of the test set for all datasets, but for Yahoo, where it turned out to be\footnote
{
Recall that on the Yahoo dataset records are discarded on the fly, so training and test set sizes are not under our full control --- see, e.g., \cite{lcls10,icml14}.
}
around 6.2\%. All experimental results reported here have been averaged over 5 runs (but in fact variance across these runs was fairly small).


\subsection{Results}
%
Our results are summarized in Figure \ref{fig:last_del}, where we report test set prediction performance. On LastFM, Delicious, and MovieLens, we measured the ratio of the cumulative regret of the algorithm to the cumulative regret of the random predictor RAN (so that the lower the better). On the Yahoo dataset, because the only available payoffs are those associated with the items recommended in the logs, we measured instead the ratio of Clickthrough Rate (CTR) of the algorithm to the CTR of RAN (so that the higher the better).
%
%
\begin{figure}[t!]
\begin{picture}(18,53)(18,53)
\begin{tabular}{l@{\hspace{-1.7pc}}l}
\includegraphics[width=0.29\textwidth]{plots/lastfm_result_100k.pdf}
& \includegraphics[width=0.29\textwidth]{plots/delicious_result_100k.pdf}\\[-1.15in]
\includegraphics[width=0.29\textwidth]{plots/movielens_result_100k_2.pdf}
& \includegraphics[width=0.29\textwidth]{plots/yahoo_result_18k.pdf}
\end{tabular}
\end{picture}
\vspace{2.05in}
\caption{\label{fig:last_del}Results on the LastFM (top left), the Delicious (top right), MovieLens (bottom left), and the Yahoo (bottom right) datasets. On the first three plots, we display the time evolution of the ratio of the cumulative regret of the algorithm (``Alg") to the cumulative regret of RAN, where ``Alg" is either ``GCLUB" (green), CLUB (blue), ``LinUCB-IND" (red), or ``LinUCB-ONE" (black). On the Yahoo dataset, we instead plot
the ratio of Clickthrough Rate (CTR) of ``Alg" to the Clickthrough Rate of RAN. Colors are consistent throughout the four plots.
}
%\vspace{-0.1in}
\end{figure}

Whereas all four datasets are generated by real online web applications, it is worth remarking that these datasets are indeed quite different in the way customers consume the associated content. For instance, the Yahoo dataset is derived from the consumption of news that are often interesting for large portions of users, hence there is no strong polarization into subcommunities (a typical ``few hits" scenario). It is thus unsurprising that on Yahoo (Lin)UCB-ONE is already doing quite well. This also explains why (Lin)UCB-IND is so poor (almost as poor as RAN). At the other extreme lies Delicious, derived from a social bookmarking web service, which is a {\em many niches} scenario. Here LinUCB-ONE is clearly underperforming. On all these datasets, CLUB performs reasonably well (this is consistent with the findings in \cite{icml14}), but in some cases the improvement over the best performer between (Lin)UCB-ONE and (Lin)UCB-IND is incremental. On LastFM, CLUB is even outperformed by LinUCB-IND in the long run. Finally, GCLUB tends to outperform all its competitors (CLUB included) in all cases.

Though preliminary in nature, we believe these findings are suggestive of two phenomena: i. building clusters over users solely based on past user behavior can be beneficial; ii. in settings of highly diverse user engagement levels (Figure \ref{fig:activity_level}), combining sequential clustering with a stochastic exploration mechanism operating at the level of cluster formation may enhance prediction performance even further.


==> implementation.tex <==


\subsection{Implementation}\label{sa:implementation}
%
As we said in the main text, in implementing the algorithm in Figure \ref{alg:club}, 
the reader should keep in mind that it is reasonable to
expect $n$ (the number of users) to be quite large, $d$ (the number of features of each item) to be relatively small,
and $m$ (the number of true clusters) to be very small compared to $n$. 
Then the algorithm can be implemented by storing a least-squares estimator $\bw_{i,t-1}$ 
at each node $i \in V$, an aggregate least squares estimator $\bbw_{\hj_t,t-1}$ for each current cluster 
$\hj_t \in \{1,\ldots, m_t\}$, and an extra data-structure which is able to perform decremental dynamic connectivity.
Fast implementations of such data-structures are those studied by~\cite{Tho97,kkm13}
(see also the research thread referenced therein). In particular, in \cite{Tho97} (Theorem 1.1 therein)
it is shown that a randomized construction exists that maintains a spanning forerst which, given an initial
undirected graph $G_1 = (V,E_1)$, is able to perform edge deletions and answer connectivity queries of the form 
``Is node $i$ connected to node $j$" in expected total time 
$O\left(\min\{|V|^2, |E_1|\,\log |V|\} + \sqrt{|V|\,|E_1|}\,\log^{2.5} |V|\right)$ for $|E_1|$ deletions. 
Connectivity queries and deletions can be 
interleaved, the former being performed in {\em constant} time. Notice that when we start off from the full graph, 
we have $|E_1| = O(|V|^2)$, so that the expected amortized time per query becomes constant. On the other hand, 
if our initial graph has
% \footnote
% {
% It is well known that a random Erdos-Renyi graph where $p = \frac{\log |V|}{|V|}$ is the independent probability that
% two nodes are connected will be a connected graph with high probability, as $|V| \rightarrow \infty$. Hence, 
% if the initial graph $G_1 = (V,E_1)$ is an Erdos-Renyi graph with $|E_1| = \Omega(|V|\,\log |V|)$, then $G_1$ 
% is likely to be a connected graph.
% } 
$|E_1| = O(|V|\,\log |V|)$ edges, then the expected amortized time per query is $O(\log^2 |V|)$. This becomes 
$O(\log^{2.5} |V|)$ if the initial graph has $|E_1| = O(|V|)$.
In addition, we maintain an $n$-dimensional vector $\ci$ containing, for each node $i \in V$, 
the index $j$ of the current cluster $i$ belongs to.

With these data-structures handy, we can implement our algorithm as follows.
% and the set of connected components of the current graph $G_t$. 
% The least-squares estimators are maintained
% by an inverse matrix $M^{-1}_{i,t}$ (or $\bM^{-1}_{j,t}$) and a vector $\bb_{i,t}$ 
After receiving $i_t$, computing $j_t$ is $O(1)$ (just by accessing $\ci$). Then, computing $k_t$ can be done
in time $O(d^2)$ (matrix-vector multiplication, executed $c_t$ times, assuming $c_t$ is a constant). 
Then the algorithm directly updates $\bb_{i_t,t-1}$ and  $\bbb_{\hj_t,t-1}$, as well
as the inverses of matrices $M_{i_t,t-1}$ and 
$\bM_{\hj_t,t-1}$, which is again $O(d^2)$, using standard formulas for rank-one adjustment of inverse matrices.
In order to prepare the ground for the subsequent edge deletion phase,
it is convenient that the algorithm also stores at each node $i$ matrix $M_{i,t-1}$ (whose time-$t$ update is again $O(d^2)$). 

Let $\delete(i,\ell)$ and $\connected(i,\ell)$ be the two operations delivered by the decremental dynamic connectivity
data-structure.
Edge deletion at time $t$ corresponds to cycling through all nodes $\ell$ such that $(i_t,\ell)$ is an existing edge.
The number of such edges is on average equal to the average degree of node $i_t$, which is $O\left(\frac{|E_1|}{n}\right)$,
where $|E_1|$ is the number of edges in the initial graph $G_1$.
Now, if $(i_t,\ell)$ has to be deleted (each the deletion test being $O(d)$), 
then we invoke $\delete(i_t,\ell)$, and then $\connected(i_t,\ell)$. If $\connected(i_t,\ell)$ = ``no", 
this means that the current cluster $\hat V_{j_t,t-1}$ has to split into two new clusters as a consequence of the 
deletion of edge $(i_t,\ell)$.
The set of nodes contained in these two clusters correspond to the two sets
%
\begin{align*}
&\{ k \in V\,:\, \connected(i_t,k) = ``yes"\},\\ 
&\{ k \in V\,:\, \connected(\ell,k) = ``yes"\}`,
\end{align*}
%
whose expected amortized computation {\em per node} is $O(1)$ to $O(\log^{2.5}n)$
(depending on the density of the initial graph $G_1$). We modify the $\ci$ vector accordingly, 
but also the aggregate least squares estimators. This is because $\bbw_{\hj_t,t-1}$ 
(represented through $\bM^{-1}_{\hj_t,t}$ and $\bbb_{\hj_t,t}$) has to be spread over the two newborn clusters.
This operation can be
performed by adding up all matrices $M_{i,t}$ and all $\bb_{i,t}$, over all $i$ belonging to each of the
two new clusters
(it is at this point that we need to access $M_{i,t}$ for each $i$),
and then inverting the resulting aggregate matrices. This operation takes $O(n\,d^2 + d^3)$.
However, as argued in the comments preceeding the statement of 
Theorem \ref{t:regret} below, with high
probability the number of current clusters $m_t$ can never exceed $m$, so that with the 
same probability this operation is only
performed at most $m$ times throughout the learning process.
Hence in $T$ rounds we have an overall (expected) running time 
%
\begin{align}
O\Biggl(&T\,\left(d^2 + \frac{|E_1|}{n}\,d\right) + m\,(n\,d^2 + d^3) + |E_1|\notag\\ 
&+ \min\{n^2, |E_1|\,\log n\} + \sqrt{n\,|E_1|}\,\log^{2.5} n\Biggl)~.\label{e:runningtime}
\end{align}
%
%where $|E_1|$ is the number of edges in the initial graph $G_1$. 
Notice that the above is $n\cdot{\mbox{poly}}(\log n)$,
if so is $|E_1|$. In addition, if $T$ is large compared to $n$ and $d$, the average running time per round
becomes $O(d^2 + d\cdot{\mbox{poly}}(\log n))$.

As for memory requirements, we need to store two $d\times d$ matrices and one $d$-dimensional 
vector at each node, one $d\times d$ matrix and one $d$-dimensional vector for each current cluster, vector 
$\ci$, and the data-structures allowing for fast deletion and connectivity tests. Overall, these data-structures 
do not require more than $O(|E_1|)$ memory to be stored, so that this implementation
takes $O(n\,d^2 + m\,d^2 + |E_1|) = O(n\,d^2+|E_1|)$, where we again relied upon the $m_t \leq m$ condition.
Again, this is $n\cdot{\mbox{poly}}(\log n)$ if so is $|E_1|$.





==> introduction.tex <==




\section{Introduction}
Exploration-exploitation techniques a.k.a. Bandits are becoming an essential tool in modern recommenders systems \cite{recsys13,recsys14}. Most recommendation setting involve an ever changing dynamic set of items, in many domains such as news and ads recommendation the item set is changing so rapidly that is impossible to use standard collaborative filtering techniques. In these settings bandit algorithms such as contextual bandits have been proven to work well \cite{lcls10} since they provide a principled way to gauge the appeal of the new items.

Yet, one drawback of contextual bandits is that they mainly work in a content-dependent regime, the user and item content features determine the preference scores so that any collaborative effects (joint user preferences over groups of items) that arise are being ignored. Incorporating collaborative effects into bandit algorithms can lead to a dramatic increase in the quality of recommendations. In bandit algorithms this has been mainly done by clustering the user. 
For instance, we may want to serve content to a group of users by taking advantage of
an underlying network of preference relationships among them. These preference relationships can either be
explicitly encoded in a graph, where adjacent nodes/users are deemed similar to one another, or implicitly
contained in the data, and given as the outcome of an inference process that recognizes similarities
across users based on their past behavior.

\sloppypar{
To deal with this issue a new type of bandit algorithms has been developed which work under the assumption that users can be grouped (or clustered) based on their selection of items e.g. \cite{icml14,cikm14}. The main assumption is that users form a graph where the edges are constructed based on signals of similar preference (e.g. a number of similar item selections). By partitioning the graphs, one can find a coherent group of users with similar preference and online behavior. While these algorithms have been proven to perform significantly better then classical contextual bandits, they "only" provide exploration on the set of items. For new users or users with sparse activity it is very difficult to find an accurate group assignment. This is a particularly important issue since most recommendation settings face unbalancedness of user activity levels, that is, relatively few users have very high activity while the vast majority of users have little to practically no activity at all (see Figure \ref{fig:activity_level} in Section \ref{s:exp}).
}

In this work, we introduce a new bandit algorithm that adds an extra exploration component over the group of users. In addition to the standard exploration-exploitation strategy over items, this algorithm explores different clustering assignments of new users and users with low activity. The experimental evaluation on four real datasets against baselines and state-of-the-art methods confirm that the additional dynamic paradigm tends to translate into solid performance benefits.


\iffalse
%

****************************

%initial draft by Shuai
Recent advances have evidently shown that exploration and exploitation is becoming a
crucial component of modern recommendation systems~\cite{recsys13,recsys14}, where if the system
designer focus on the user preference partially only, it would lead to quite a few same recommendations
for all users. Which naturally urges us to consider the ever-changing content universe took into account
in the highly dynamic environment.
On the other hand, users or customers always have strong desire of knowing the future, it's the future it
matters based on the learning experience from the past. That is, life can only be understood backwards,
but it must be lived forwards [Quote of Soren Kierkegaard]. Hence this paper tries to provide a principal
online prediction solution for recommender systems based on the graph clustering idea~\cite{pami07,sigkdd05}
augmented by the multi-armed bandits framework. More concretely, standing on the shoulder of bleeding-edge machine
learning model~\cite{icml14}, we carefully elaborate and import the training stage boosted mechanism, whereas
~\cite{icml14} treats each user equally likely. And it turns our our machinery not only faster in the scalable sense
where for the large number of users is our key concern, but also achieves significant improved performance
in terms of prediction accuracy compared to several state-of-the-art bandit methods.




%
%\vspace{-0.05in}
Presenting personalized content to users is nowdays a crucial functionality for many online
recommendation services. Due to the ever-changing set of available options, these services
have to exhibit strong adaptation capabilities when trying to match
%as much as possible the
users' preferences.
%In essence,
Coarsely speaking, the underlying systems repeatedly learn a mapping between available content
and users, the mapping being based on {\em context} information (that is, sets of features) which is
typically extracted from both users and contents.
The need to focus on content that raises the users' interest,
combined with the need of exploring new content so as to globally improve users' experience,
generates a well-known exploration-exploitation dilemma, which is commonly formalized as
a multi-armed bandit problem~(e.g., \cite{lr85,ACF01,audibert:hal-00711069,CaronKLB12}).
In particular, the contextual bandit methods~(e.g., \cite{Aue02,lz07,li2010contextual,chu2011contextual,
bogers2010movie,abbasi2011improved,cg11,ko11,salso11,yhg12,dkc13}, and references therein)
have rapidly become a reference algorithmic technique for implementing adaptive recommender systems.

%\vspace{-0.05in}
% new challenge: users are increasing in number, and interact
Within the above scenarios, the widespread adoption of online social networks, where users are
engaged in technology-mediated social interactions (making product endorsement and word-of-mouth
advertising a common practice), raises further challenges and opportunities to content recommendation
systems: On one hand, because of the mutual influence among friends, acquaintances, business partners,
etc., users having strong ties are more likely to exhibit similar interests, and therefore similar
behavior. On the other hand, the nature and scale of such interactions calls for adaptive
algorithmic solutions which are also computationally affordable.

%\vspace{-0.05in}
% two approaches: explicit networks and implicit networks
Incorporating social components into bandit algorithms can lead to a dramatic increase in the quality
of recommendations. For instance, we may want to serve content to a group of users by taking advantage of
an underlying network of social relationships among them. These social relationships can either be
explicitly encoded in a graph, where adjacent nodes/users are deemed similar to one another, or implicitly
contained in the data, and given as the outcome of an inference process that recognizes similarities
across users based on their past behavior.
Examples of the first approach are the recent works~\cite{bes13,dkmc13,cgz13}, where
a social network structure over the users is assumed to be given that reflects actual interest similarities
among users -- see also \cite{cb13, valko2014spectral} for recent usage of social information to tackle the so-called
``cold-start" problem. Examples of the second approach are the more traditional
collaborative-filtering (e.g.,~\cite{skr99}), content-based filtering, and hybrid approaches (e.g.~\cite{b05}).

Both approaches have important drawbacks hindering their practical deployment. One obvious drawback
of the ``explicit network" approach is that the social network information may be misleading
%(e.g., ``is it really true that if we are friends in Facebook then we like the same books ?")
(see, e.g., the experimental evidence reported by~\cite{dkmc13}), or simply unavailable.
Moreover, even in the case when this information is indeed available and useful,
the algorithmic strategies to implement the needed feedback sharing mechanisms might lead to severe
scaling issues~\cite{cgz13}, especially when the number of targeted users is large.
A standard drawback of the ``implicit network" approach of traditional recommender systems
is that in many practically relevant scenarios (e.g., web-based), content universe and popularity often
undergo dramatic changes, making these approaches difficult to apply.

%\vspace{-0.05in}
In such settings, most notably in the relevant case
when the involved users are many, it is often possible to identify
a few subgroups or communities within which users share similar interests~\cite{rlkr06,bwdh12},
%~\cite{xlyxzyc05,rlkr06,bwdh12},
thereby greatly facilitating
the targeting of users by means of {\em group} recommendations. Hence the system need not learn
a different model for each user of the service, but just a single model for each group.

%\vspace{-0.05in}
In this paper, we carry out\footnote
{
Due to space limitations, we postpone the discussion of related work to the supplementary
material.
}
%\footnote
%{
%The only paper we are aware of which has similar goals as ours is~\cite{bkm12}, though that
%paper apparently works under more restrictive assumptions.
%}
a theoretical and experimental investigation of adaptive clustering algorithms
for linear (contextual) bandits under the assumption that we have to serve content to a set of $n$ users
organized into $m << n$ groups (or {\em clusters}) such that users within each group tend to provide
similar feedback to content recommendations. We give a $O(\sqrt{T})$ regret analysis holding in a standard
stochastically linear setting for payoffs where, importantly, the hidden constants in the big-oh
depend on $m$, rather than $n$, as well as on the geometry of the user models within the different
clusters.
%
The main idea of our algorithm is to use confidence balls of the users' models to both estimate user similarity,
and to share feedback across (deemed similar) users. The algorithm adaptively interpolates between
the case when we have a single instance of a contextual bandit algorithm making the same predictions for all
users and the case when we have $n$-many instances providing fully personalized recommendations.
We show that our algorithm can be implemented efficiently (the large $n$ scenario being of special concern here)
by means of off-the-shelf data-structures relying on random graphs. Finally, we test our algorithm
on medium-size synthetic and real-world datasets, often reporting a significant increase in prediction performance
over known state-of-the-art methods for bandit problems.

\iffalse
In practice, it is often the case that the system does not need to learn a different model for each single user of the service, but it can just learn a model for each cluster of users with similar taste.
This problem has somehow already been addressed in previous papers, assuming that side information from a social network among the users was provided to the algorithm (i.e., see \cite{}).
Unfortunately, it is not always the case: in some cases there is not information available about the users except their current behavior, and even when the side information is available it may not provide good similarity information. %This will also address the problem of learning personalized models when the users interact with the service very few times.
Learning the similarity among the users while learning their preferences model is far from trivial.\\
In this work, we provide an algorithm for contextual bandits able to learn and leverage the similarity among the users.

The main idea is to use the confidence balls of the users' models to estimate the similarity among the users and in this way allow the algorithm to share feedback among similar users.
This mechanism is implemented running a single contextual bandit algorithm for each cluster of users, using all the feedback obtained for all the predictions made for the users in the cluster.
Roughly speaking, the algorithm interpolates between the case where there is only one instance of a contextual bandits making predictions for all the users and the case where there is a single instance of a contextual bandit algorithm for each user.\\
In the last part of the paper, we present a comparison between the new algorithm and the state of the art linear bandit algorithms in a completely controlled environment.
Oftentimes our algorithm outperforms its competitors and it is never worse than the best among them.
{\bf CG: say upfront that we face the unbalancedness of user activity levels}

\fi

\fi


==> learning_and_alg.tex <==

\vspace{-0.07in}
\section{Learning Model}\label{s:model}
%
\vspace{-0.05in}
We assume the user behavior similarity %over the social network
is encoded as
an {\em unknown} clustering of the users. Specifically, let
$V = \{1,\ldots, n\}$ represent the set of $n$ users. Then $V$ can be partitioned
into a small number $m$ of clusters $V_1, V_2, \ldots, V_m$, with $m << n$, such that
users lying in the same cluster share similar behavior and users lying in different
clusters have %significantly
different behavior. The actual partition of $V$
(including the number of clusters $m$) and the common user behavior within each
cluster are unknown to the learner, and have to be inferred on the fly.

\vspace{-0.05in}
Learning proceeds in a sequential fashion: At each round $t=1,2,\dots$,
the learner receives a user index $i_t \in V$ together with a set of
context vectors $C_{i_t} = \{\bx_{t,1}, \bx_{t,2},\ldots, \bx_{t,c_t}\} \subseteq \R^d$.
The learner then selects some ${\bar \bx_t} =  \bx_{t,k_t} \in C_{i_t}$ to recommend to user $i_t$,
and observes some payoff $a_t \in \R$, which is a function of both $i_t$ and the recommended
${\bar \bx_t}$.
%
The following assumptions are made on how index $i_t$, set $C_{i_t}$, and payoff $a_t$
are generated in round $t$. Index $i_t$ represents the user to be served by the system,
and we assume $i_t$ is selected uniformly at random\footnote
{
Any other distribution that insures a positive probability of visiting each node of $V$ would suffice here.
}
from $V$. Once $i_t$ is selected,
the number of context vectors $c_t$ in $C_{i_t}$
is generated arbitrarily as a function of past indices $i_1, \ldots, i_{t-1}$, payoffs $a_1, \ldots, a_{t-1}$,
and sets $C_{i_1}, \ldots, C_{i_{t-1}}$, as well as the current index $i_t$.
Then
the sequence $\bx_{t,1}, \bx_{t,2},\ldots, \bx_{t,c_t}$ of context vectors
within $C_{i_t}$
% (as well as the number $c_t$ of its elements) is generated
% arbitrarily as a function of past indices $i_1, \ldots, i_{t-1}$, rewards $a_1, \ldots, a_{t-1}$,
% and sets $C_{i_1}, \ldots, C_{i_{t-1}}$, as well as the current index $i_t$.
%
is generated i.i.d. (conditioned on $i_t, c_t$ and all past indices $i_1, \ldots, i_{t-1}$,
payoffs $a_1, \ldots, a_{t-1}$, and sets $C_{i_1}, \ldots, C_{i_{t-1}}$)
from a random process on the surface of the unit sphere,
whose process matrix $\E[XX^\top]$ is full rank, with minimal eigenvalue $\lambda > 0$.
Further assumptions on the process matrix $\E[XX^\top]$ are made later on.
%
Finally, payoffs are generated by noisy versions of unknown linear functions
of the context vectors. That is, we assume each cluster $V_j$, $j = 1, \ldots, m$,
hosts an unknown parameter vector $\bu_j \in \R^d$ which is common to each user $i \in V_j$.
Then the payoff value
$a_i(\bx)$ associated with user $i$ and context vector $\bx \in \R^d$ is given by the random variable
\[
a_i(\bx) = \bu_{j(i)}^\top\bx + \epsilon_{j(i)}(\bx)~,
\]
where $j(i) \in \{1, 2, \ldots, m\}$ is the index of the cluster that node $i$ belongs to, and
$\epsilon_{j(i)}(\bx)$ is a conditionally zero-mean and bounded variance noise term.
%
Specifically, denoting by $\E_t[\,\cdot\,]$ the conditional expectation\
\(
\E\bigl[\,\cdot\,\big|\, (i_1, C_{i_1}, a_1), \ldots, (i_{t-1}, C_{i_{t-1}}, a_{t-1}), i_t\,\bigr],
\)
% \ we take the general approach of \cite{abbasi2011improved},
% and 
we assume that for any fixed $j \in \{1,\ldots,m\}$ and $\bx \in \R^d$, the variable
$\epsilon_j(\bx)$ is such that
% conditionally sub-Gaussian with variance parameter $\sigma^2 > 0$, namely,
% $\E_t\bigl[\exp(\gamma\,\epsilon_j(\bx))|\,\bx\,\bigr] \leq \exp\bigl(\sigma^2\,\gamma^2/2\bigr)$
% for all $\gamma \in \R$ and all $\bx,v$.
% This implies 
$\E_t[\epsilon_{j}(\bx)|\,\bx\,] = 0$ and
$\Var_t\bigl[\epsilon_{j}(\bx)|\,\bx\,\bigr] \leq \sigma^2$, where $\Var_t[\,\cdot\,]$ is
a shorthand for the conditional variance
$
\Var\bigl[\,\cdot\,\big|\, (i_1, C_{i_1}, a_1), \ldots, (i_{t-1}, C_{i_{t-1}}, a_{t-1}),i_t\,\bigr]
$
of the variable at argument.
So we clearly have $\E_t[a_i(\bx)|\,\bx\,] = \bu_{j(i)}^\top\bx$ and
$\Var_t\bigl[a_i(\bx)|\,\bx\,\bigr] \leq \sigma^2$.
Therefore, $\bu_{j(i)}^\top\bx$ is the expected payoff observed at user $i$
for context vector $\bx$. %(e.g., the click rate of user $i$ on the ad encoded by $\bx$).
In the special case when the noise
$\epsilon_{j(i)}(\bx)$ is a bounded random variable taking values in the range
$[-1,1]$, this implies $\sigma^2 \leq 1$. We will make throughout the assumption that
$a_i(\bx) \in [-1,1]$ for all $i \in V$ and $\bx$. Notice that this implies
$-1 \leq \bu_{j(i)}^\top\bx \leq 1$ for all $i \in V$ and $\bx$.
Finally, we assume well-separatedness among the clusters, in that\
\(
||\bu_{j}-\bu_{j'}|| \geq \gamma > 0\ {\mbox{for all $j \neq j'$}}.
\)
\ We define the regret $r_t$ of the learner at time $t$ as
%
% the extent to which
% the average payoff of the best choice in hindsight at user $i_t$ exceeds the average payoff
% of the algorithm's choice, i.e.,
\vspace{-0.05in}
\[
r_t = \left(\max_{\bx \in C_{i_t} }\, \bu_{j(i_t)}^\top\bx\right) - \bu_{j(i_t)}^\top{\bar \bx_{t}}~.
\]
We are aimed at bounding with high probability (over the variables $i_t$,
$\bx_{t,k}$, $k = 1,\ldots, c_t$,
and the noise variables $\epsilon_{j(i_t)}$) the cumulative regret
\(
\sum_{t=1}^T r_t~.
\)
The kind of regret bound we would like to obtain (we call it the {\em reference} bound) is one where
the clustering structure of $V$ (i.e., the partition of $V$ into $V_1, \ldots, V_m$) is known to the algorithm
ahead of time, and we simply view each one of the $m$ clusters as an independent bandit problem.
%
In this case, a standard contextual bandit analysis \cite{Aue02,chu2011contextual,abbasi2011improved}
shows that, as $T$ grows large, the cumulative
regret $\sum_{t=1}^T r_t$ can be bounded with high probability as\footnote
{
The ${\tilde O}$-notation hides logarithmic factors.
}
\vspace{-0.05in}
%\[
\begin{center}
\(
\sum_{t=1}^T r_t
=
{\tilde O}\Bigl(\sum_{j = 1}^m \left(\sigma\,d + ||\bu_j||\,\sqrt{d}\right)\,\sqrt{T}\Bigl)~.
\)
\end{center}
%\]
%with high probability.
% at least $1-\delta$.
% where
% \[
% L(\bu_1, \ldots, \bu_m) = \sum_{i = 1}^m ||\bu_i||^2
% \]
% encodes the ``complexity" of the parametric inference problem. Notice that
% $L(\bu_1, \ldots, \bu_m)$ is supposed to be small, since so is $m$ (compared to $n$).
%
For simplicity, we shall assume that $||\bu_j|| = 1$ for all $j = 1, \ldots, m$. Now,
a more careful analysis exploiting our assumption about the randomness of $i_t$ (see the supplementary
material) reveals that one can replace
the $\sqrt{T}$ term contributed by each bandit $j$ by a term of the form
$\sqrt{T}\,\left(\frac{1}{m}+\sqrt{\frac{|V_j|}{n}}\right)$, so that
under our assumptions the reference bound becomes
%
\vspace{-0.02in}
\begin{equation}\label{e:referencebound}
\sum_{t=1}^T r_t
=
{\tilde O}\Biggl(\left(\sigma\,d + \sqrt{d}\right)\sqrt{T}\Bigl(1+\sum_{j=1}^m \sqrt{\frac{|V_j|}{n}}\Bigl)\Biggl)~.
\end{equation}
%\vspace{-0.05in}
%
%$L(\bu_1, \ldots, \bu_m) = m$.
Observe the dependence of this bound on the size of clusters $V_j$. The worst-case scenario is when
we have $m$ clusters of the same size $\frac{n}{m}$, resulting in the bound
%
\vspace{-0.08in}
%\[
\begin{center}
\(
\sum_{t=1}^T r_t
=
{\tilde O}\left(\left(\sigma\,d + \sqrt{d}\right)\,\sqrt{m\,T}\right)~.
\)
\end{center}
%\]
%\vspace{-0.05in}
%
At the other extreme lies the easy case when we have a single big cluster and many small ones.
For instance, $|V_1| = n-m+1$, and $|V_2| = |V_3| = \ldots |V_m| = 1$, for $m << n$, gives
\vspace{-0.05in}
%\[
\begin{center}
\(
\sum_{t=1}^T r_t
=
{\tilde O}\Bigl(\left(\sigma\,d + \sqrt{d}\right)\,\sqrt{T}\,\Bigl(1+\frac{m}{\sqrt{n}}\Bigl)\Bigl)~.
\)
\end{center}
%\]
%\vspace{-0.05in}
%
A relevant geometric parameter of the set of $\bu_j$ is the {\em sum of distances}
$SD(\bu_j)$ of a given vector $\bu_j$
%$R$
w.r.t. the set of vectors $\bu_1, \ldots, \bu_m$,
%w.r.t. among them,
which we define as\
\(
SD(\bu_j) = \sum_{\ell = 1}^m ||\bu_j - \bu_{\ell}||.\
%R = \frac{1}{n}\max_{i,j = 1,\ldots, m} ||\bu_i - \bu_j||~,
\)
%i.e., the maximal distance of $\bu_i$ to all other vectors.
%
If it is known that $SD(\bu_j)$ is small for all $j$, one can modify the abovementioned
independent bandit algorithm, by letting the bandits share signals,
as is done, e.g., in \cite{cgz13}. This allows one to exploit the vicinity of the $\bu_j$ vectors,
and roughly replace
\(
1+\sum_{j=1}^m \sqrt{\frac{|V_j|}{n}}
\)
in (\ref{e:referencebound}) by a quantity also depending on the mutual distances
$||\bu_j - \bu_{j'}||$ among cluster vectors.
However, this improvement is obtained at the cost of a substantial increase of running time \cite{cgz13}.
%
In our analysis (Theorem \ref{t:regret} in Section \ref{s:alg}), we would like to leverage both
%the payoff noise model and
the geometry of the clusters, as encoded by vectors $\bu_j$, and the
relative size $|V_j|$ of the clusters, with no prior knowledge of $m$ (or $\gamma$), and
without too much extra computational burden.



\vspace{-0.1in}
\section{The Algorithm}\label{s:alg}
%
\vspace{-0.05in}
Our algorithm, called Cluster of Bandits (CLUB), is described in Figure \ref{alg:club}.
In order to describe the algorithm
%(and its subsequent analysis in Section \ref{s:analysis}),
we find it convenient to re-parameterize the problem described in Section \ref{s:model},
and introduce $n$ parameter vectors $\bu_1, \bu_2, \ldots, \bu_n$, one per node, where nodes
within the same cluster $V_j$ share the same vector. An illustrative example is given in
Figure \ref{f:1}.

\vspace{-0.05in}
The algorithm maintains at time $t$ an estimate $\bw_{i,t}$ for
vector $\bu_i$ associated with user $i \in V$. Vectors $\bw_{i,t}$ are updated based
on the payoff signals, similar to a standard linear bandit algorithm
(e.g.,~\cite{chu2011contextual}) operating on the context vectors contained in
$C_{i_t}$. Every user $i$ in $V$ hosts a linear bandit algorithm
like the one described in \cite{cgz13}.
%In fact there are two versions of these weight estimates: one is $\bw'_{i,t}$, the other is
%$\bw_{i,t}$. The former is just an intermediate version, the latter being the
%projection of the former into the unit ball with respect to the Mahalanobis distance
%$d_{i,t}(\bw,\bw') = (\bw - \bw') M_{i,t} (\bw - \bw')$.
One can see that the
%intermediate
prototype vector $\bw_{i,t}$ is the result of a standard linear least-squares
approximation to the corresponding unknown parameter vector $\bu_i$.
In particular, $\bw_{i,t-1}$ is defined through the inverse correlation matrix $M^{-1}_{i,t-1}$,
and the additively-updated vector $\bb_{i,t-1}$.
Matrices $M_{i,t}$ are initialized to the $d\times d$ identity matrix,
and vectors $\bb_{i,t}$ are initialized to the $d$-dimensional zero vector.
In addition, the algorithm maintains at time $t$ an undirected
graph $G_t = (V,E_t)$ whose nodes are precisely the users in $V$. The algorithm starts off from the complete
graph, and progressively erases edges based on the evolution of vectors $\bw_{i,t}$. The graph is intended
to encode the current partition of $V$ by means of the {\em connected components} of $G_t$.
We denote by $\hat V_{1,t}, \hat V_{2,t}, \ldots, \hat V_{m_t,t}$ the partition of $V$ induced by the connected
components of $G_t$. Initially, we have $m_1 = 1$ and
$\hat V_{1,1} = V$. The clusters $\hat V_{1,1}, \hat V_{2,t}, \ldots, \hat V_{m_t,t}$
(henceforth called the {\em current} clusters)
are indeed meant to estimate the underlying true partition $V_1, V_2, \ldots, V_{m}$, henceforth called
the {\em underlying} or {\em true} clusters.
%, and have corresponding {\em representative} nodes $\hs_{1,t}, \hs_{2,t}, \ldots, \hs_{m_t,t} \in V$
% with associated weight vectors
% $\bw_{\hs_{1,t},t}, \bw_{\hs_{2,t},t}, \ldots, \bw_{\hs_{m_t,t},t}$.
% taken from among $\bw_{1,t}, \ldots, \bw_{n,t}$.

%
\begin{figure}[t!]
\begin{center}
\begin{algorithmic}
\small
%\vspace{-1.4in}
\STATE \textbf{Input}: Exploration parameter $\alpha > 0$; edge deletion parameter $\alpha_2 > 0$; probability parameter $\rho < 1/2$
\STATE \textbf{Init}:
\vspace{-0.1in}
\begin{itemize}
\item $\bb_{i,0} = \bzero \in \R^d$ and $M_{i,0} = I \in \R^{d\times d}$,\ \ $i = 1, \ldots n$;
\vspace{-0.1in}
\item Clusters ${\hat V_{1,1}} = V$, number of clusters $m_1 = 1$;
\vspace{-0.1in}
\item Graph $G_1 = (V,E_1)$, $G_1$ is connected over $V$.
\end{itemize}
\vspace{-0.1in}
\FOR{$t =1,2,\dots,T$}
\STATE Receive $i_t \in V$;
\IF {$t \leq T \times 20\%$}
	\STATE With probability $\rho$ conduct the cold start training boosted exploration: pick one cluster uniformly at random, execute one fast graph clustering procedure and delete edges correspondingly by ending up with one more clusters;%the fast graph (mincut-like) clustering tool: graclus
	%\STATE With high probability $\rho$ locate the cluster that current served user $i_t$ belongs to, within that cluster find the $i_t$'s neighborhood set that made up of directed connected user, delete the edges among them
\ENDIF 
%\COMMENT{This is a comment statement}
\STATE Set $\bw_{i,t-1} = M_{i,t-1}^{-1}\bb_{i,t-1}$, \quad $i = 1, \ldots, n$;
\STATE Get context
       $
       C_{i_t} = \{\bx_{t,1},\ldots,\bx_{t,c_t}\};
       $
\STATE Determine $\hj_t \in \{1, \ldots, m_t\}$ such that $i_t \in {\hat V_{\hj_t,t}}$, and set
\vspace{-0.1in}
\begin{align*}
   \bM_{{\hj_t},t-1}  &= I+\sum_{i \in {\hat V_{\hj_t,t}}} (M_{i,t-1}-I),\\
   \bbb_{{\hj_t},t-1} &= \sum_{i \in {\hat V_{\hj_t,t}}} \bb_{i,t-1},\\
   \bbw_{{\hj_t},t-1} &= \bM_{{\hj_t},t-1}^{-1}\bbb_{{\hj_t},t-1}~;
\end{align*}
\vspace{-0.4in}
%\STATE Set $\bw'_{\hs_t,t-1} = M_{\hs_t,t-1}^{-1}\,\bb_{\hs_t,t-1}$;
%\STATE Set, for all $i \in V$,
%       \[
%       \bw_{i,t-1} = \arg\min_{\bw \in \R^d\,:\, ||\bw||=1} d_{i,t-1}(\bw,\bw'_{i,t-1}),
%       \]
%       where
%       \[
%       d_{i,t}(\bw,\bw') = (\bw-\bw')^\top M_{i,t}(\bw-\bw');
%       \]
\STATE \[
       {\mbox{Set\ \ }}
        k_t = \argmax_{k = 1, \ldots, c_t} \left({\bbw_{\hj_t,t-1}}^\top\bx_{t,k}  + \CB_{\hj_t,t-1}(\bx_{t,k})\right),
       \]
\vspace{-0.2in}
       \begin{align*}
       \CB_{j,t-1}(\bx) &= \alpha\,\sqrt{\bx^\top \bM_{j,t-1}^{-1} \bx\,\log(t+1)},\\%\ j = 1, \ldots, m_t~,
       \bM_{j,t-1} &= I+\sum_{i \in {\hat V_{j,t}}} (M_{i,t-1}-I)\,,\quad j = 1, \ldots, m_t~.
       \end{align*}
%       and
%       \[
%         \clip(x) =
%         \begin{cases}
%           1 & {\mbox{\ If $ x > 1$,}}\\
%           x & {\mbox{\ If $ -1 \leq x \leq 1$,}}\\
%          -1 & {\mbox{\ If $ x < -1$;}}
%         \end{cases}
%       \]
\vspace{-0.1in}
\STATE Observe payoff $a_t \in [-1,1]$;
\STATE Update weights:
       \begin{itemize}
       \vspace{-0.1in}
       \item $M_{i_t,t} = M_{i_t,t-1} + {\bar \bx_{t}}{\bar \bx_{t}}^\top$,
       \vspace{-0.1in}
       \item $\bb_{i_t,t} = \bb_{i_t,t-1} + a_t {\bar \bx_t}$,
       \vspace{-0.1in}
       \item Set $M_{i,t} =  M_{i,t-1},\ \bb_{i,t} = \bb_{i,t-1}$ for all $i \neq i_t$~;
       \end{itemize}
\STATE Update clusters:
       \begin{itemize}
       \vspace{-0.1in}
       \item Delete from $E_t$ all $(i_t,\ell)$ such that
       \[
             ||\bw_{i_t,t-1} - \bw_{\ell,t-1}|| > \sCB_{i_t,t-1} + \sCB_{\ell,t-1}~,
       \]
%      where
       \vspace{-0.3in}
       \begin{align*}
        \sCB_{i,t-1} &= \alpha_2\,\sqrt{\frac{1+\log(1+T_{i,t-1})}{1+T_{i,t-1}}},\\
        T_{i,t-1}    &= |\{s \leq t-1\,:\, i_s = i \}|,\qquad i \in V;
       \end{align*}
       \vspace{-0.3in}
       \item Let $E_{t+1}$ be the resulting set of edges, set $G_{t+1} = (V,E_{t+1})$,
        and compute associated clusters
        $\hat V_{1,t+1}, \hat V_{2,t+1}, \ldots, \hat V_{m_{t+1},t+1}$~.
       \end{itemize}
\ENDFOR
\end{algorithmic}
\vspace{-0.1in}
\caption{\label{alg:club}
Pseudocode of the GCLUB algorithm.
The confidence functions $\CB_{j,t-1}$ and $\sCB_{i,t-1}$ are simplified versions of
their ``theoretical" counterparts $\TCB_{j,t-1}$ and $\sTCB_{i,t-1}$, defined later on.
The factors $\alpha$ and $\alpha_2$ are used here as tunable parameters that bridge the simplified
versions to the theoretical ones.
\vspace{-0.25in}
}
\end{center}
\end{figure}
%
%
%copied and modified in order to save space
%most of the content is already written in other parts of the paper
%
\vspace{-0.05in}
At each time $t=1,2,\dots$, the algorithm receives the index $i_t$ of the user to serve, and the
associated context vectors $\bx_{t,1}, \ldots, \bx_{t,c_t}$
(the set $C_{i_t}$), and must select one among them. In doing so, the algorithm first determines
which cluster (among $\hat V_{1,1}, \hat V_{2,t}, \ldots, \hat V_{m_t,t}$)
node $i_t$ belongs to, call this cluster $\hat V_{\hj_t,t}$,
then builds the aggregate weight vector $\bbw_{\hj_t,t-1}$ by taking prior ${\bar \bx_s}$, $s < t$,
such that $i_s \in \hat V_{\hj_t,t}$, and computing the least squares approximation as if all nodes
$i \in \hat V_{\hj_t,t}$ have been collapsed into one.
%
\iffalse
***************************************************
%CG: commented out due to lack of space
, that is,
%
\vspace{-0.1in}
\begin{eqnarray*}
\bM_{\hj_t,t-1} &=& I + \sum_{s < t\,:\, i_s \in {\hat V_{\hj_t,t}}} {\bar \bx_s}{\bar \bx_s}^\top,\\
\bbb_{\hj_t,t-1} &=& \sum_{s < t\,:\, i_s \in {\hat V_{\hj_t,t}}} a_s\,{\bar \bx_s},\\
\bbw_{{\hj_t},t-1} &=& \bM_{{\hj_t},t-1}^{-1}\bbb_{{\hj_t},t-1}~.
\end{eqnarray*}
%\vspace{-0.1in}
%
Notice that the above definition of $\bM_{\hj_t,t-1}$
is equivalent to the one given in Figure \ref{alg:club}.
***************************************************
\fi
%
It is weight vector $\bbw_{{\hj_t},t-1}$ that the algorithm uses to select $k_t$.
In particular,
% the representative $\hs_{t}$ is computed as\footnote
% {
% Ties are broken in some deterministic way, e.g., by smallest node index.
% }
% \[
%          \hs_t = \arg\min_{v \in {\hat V_{j,t}}} \sCB_{v,t-1}~,
% \]
% where
% \[
%         \sCB_{i,t} = \alpha\,\sqrt{\frac{1+\log(1+T_{i,t})}{1+T_{i,t}}},\qquad i \in V~,
% \]
% being
% \[
% T_{i,t} = |\{s \leq t\,:\, i_s = i\}|
% \]
% the number of rounds up to time $t$ that node $i$ was requested.
% \[
% \hs_t = \argmax_{v \in \hat V_{j,t}} T_{v,t-1}~,
% \]
% i.e., $\hs_t$ is the node that has so far being served most often, among the nodes in the
% current cluster that $i_t$ belongs to.
% Notice that this definition of $\hs_t$ is equivalent to the one in CLUB's pseudocode,
% since the function $x\,:\, \rightarrow \frac{1+\log(1+x)}{1+x}$ is monotonically decreasing in $x \geq 0$.
% Moreover,
\vspace{-0.04in}
\[
       k_t = \argmax_{k = 1, \ldots, c_t} \left({\bbw_{\hj_t,t-1}}^\top\bx_{t,k}  + \CB_{\hj_t,t-1}(\bx_{t,k})\right)~.
\]
%with
% \vspace{-0.05in}
% \[
%        \CB_{j,t-1}(\bx) = \alpha\,\sqrt{\bx^\top \bM_{j,t-1}^{-1} \bx\,\log(t+1)}\,,\, j = 1, \ldots, m_t~,
% \]
% where\ \
% \(
%         \bM_{j,t-1} = I+\sum_{i \in {\hat V_{j,t}}} (M_{i,t-1}-I),\ \ j = 1, \ldots, m_t,\ \
% \)
% is the aggregate matrix associated with (current) cluster $j$.
The quantity $\CB_{\hj_t,t-1}(\bx)$ is a version of the upper confidence bound in the approximation of
$\bbw_{\hj_t,t-1}$ to a suitable combination
of vectors $\bu_i$, $i \in {\hat V_{\hj_t,t}}$ -- see the supplementary material for details.
%, as well as Figure \ref{f:1}.

\vspace{-0.05in}
Once this selection is done and the associated payoff $a_t$ is observed, the algorithm uses the selected vector
${\bar \bx_t}$ for updating $M_{i_t,t-1}$ to $M_{i_t,t}$ via a rank-one adjustment,
and for turning vector $\bb_{i_t,t-1}$ to $\bb_{i_t,t}$
via an additive update whose learning rate is precisely $a_t$.
Notice that the update is only performed at node $i_t$, since for all other $i \neq i_t$ we have
$\bw_{i,t} = \bw_{i,t-1}$. However, this update at $i_t$ will also implicitly update the
aggregate weight vector $\bbw_{\hj_{t+1},t}$ associated with cluster ${\hat V_{\hj_{t+1},t+1}}$ that node $i_t$
will happen to belong to in the next round.
% not at node $\hs_t$.
%
Finally, the cluster structure is possibly modified. At this point
CLUB compares, for all existing edges $(i_t,\ell) \in E_{t}$, the distance
\(
||\bw_{i_t,t-1}- \bw_{\ell,t-1}||
\)
between
%the projected
vectors $\bw_{i_t,t-1}$ and $\bw_{\ell,t-1}$
to the quantity
\(
\sCB_{i_t,t-1} + \sCB_{\ell,t-1}~.
\)
If the above distance is significantly large (and $\bw_{i_t,t-1}$ and $\bw_{\ell,t-1}$ are good approximations to
the respective underlying vectors $\bu_{i_t}$ and $\bu_{\ell}$),
%
% then we expect that both $\sCB_{i_t,t}$ and
% $\sCB_{j,t}$ are small, making
%
then this is a good indication that
$\bu_{i_t} \neq \bu_{\ell}$ (i.e., that node $i_t$ and node $\ell$ cannot belong to the same true cluster), so that
edge $(i_t,\ell)$ gets deleted.
The new graph $G_{t+1}$, and the induced partitioning clusters $\hat V_{1,t+1}, \hat V_{2,t+1}, \ldots, \hat V_{m_{t+1},t+1}$,
%and associated representatives $\hs_{1,t+1}, \hs_{2,t+1}, \ldots, \hs_{m_{t+1},t+1}$
are then computed, and a new round begins.


\iffalse
***************************************************************
At each time $t=1,2,\dots$, the algorithm receives the index $i_t$ of the user to serve, and the
associated context vectors $\bx_{t,1}, \ldots, \bx_{t,c_t}$
(the set $C_{i_t}$), and must select one among them. In doing so, the algorithm first determines
which cluster node $i_t$ belongs to, among those available at time $t$,
and then builds the aggregate weight vector
$\bbw_{\hj_t,t-1}$ by taking prior ${\bar \bx_s}$, $s < t$


belonging to the users in cluster and


computing the least squares approximation as if all nodes
$i \in \hat V_{\hj_t,t}$ have been collapsed into one.

The quantity
$\CB_{\hj_t,t-1}(\bx)$ is a version of the upper confidence bound in the approximation of
$\bbw_{\hj_t,t-1}$ to a suitable combination
of vectors $\bu_i$, $i \in {\hat V_{\hj_t,t}}$ -- see Lemma \ref{l:comboapprox} in the supplementary
material.

Once this selection is done and the associated payoff $a_t$ is observed, the algorithm uses the selected vector
${\bar \bx_t}$ for updating $M_{i_t,t-1}$ to $M_{i_t,t}$ via a rank-one adjustment,
and for turning vector $\bb_{i_t,t-1}$ to $\bb_{i_t,t}$
via an additive update whose learning rate is precisely $a_t$.
Notice that the update is only performed at node $i_t$, since for all other $i \neq i_t$ we have
$\bw_{i,t} = \bw_{i,t-1}$. However, this update at $i_t$ will also implicitly update the
aggregate weight vector $\bbw_{\hj_{t+1},t}$ associated with cluster ${\hat V_{\hj_{t+1},t+1}}$ that node $i_t$
will happen to belong to in the next round.
% not at node $\hs_t$.

Finally, the cluster structure is possibly modified:
CLUB compares, for any existing edge $(i_t,\ell) \in E_{t}$, the distance
\(
||\bw_{i_t,t-1}- \bw_{\ell,t-1}||
\)
between
%the projected
vectors $\bw_{i_t,t-1}$ and $\bw_{\ell,t-1}$
to the quantity
\(
\sCB_{i_t,t-1} + \sCB_{\ell,t-1}~.
\)
If the above distance is significantly large (and $\bw_{i_t,t-1}$ and $\bw_{\ell,t-1}$ are good approximations to
the respective underlying vectors $\bu_{i_t}$ and $\bu_{\ell}$),
%
% then we expect that both $\sCB_{i_t,t}$ and
% $\sCB_{j,t}$ are small, making
%
then this is a good indication that
$\bu_{i_t} \neq \bu_{\ell}$ (i.e., that node $i_t$ and node $\ell$ cannot belong to the same true cluster), so that
edge $(i_t,\ell)$ gets deleted.
The new graph $G_{t+1}$, and the induced partitioning clusters $\hat V_{1,t+1}, \hat V_{2,t+1}, \ldots, \hat V_{m_{t+1},t+1}$,
%and associated representatives $\hs_{1,t+1}, \hs_{2,t+1}, \ldots, \hs_{m_{t+1},t+1}$
are then computed, and a new round begins.
****************************************************
\fi




==> macros.tex <==

\iffalse
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{definition}[theorem]{Definition}
\fi

\newtheorem{claim}{Claim}
\newtheorem{remark}{Remark}

\newcommand{\cN}{\mathcal{N}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\hrangle}{\rangle_{\mathbb{H}}}

\newcommand{\cF}{\mathcal{F}}
\newcommand{\into}{\rightarrow}
\newcommand{\eqc}{\doteqdot}
\newcommand{\neqc}{\not\doteqdot}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cL}{\mathcal{L}}

\newcommand{\bbN}{\mathbb{N}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Var}{\mathbb{V}}
\newcommand{\br}{\mathbf{r}}
\newcommand{\bi}{\mathbf{i}}
\newcommand{\cut}{\phi}

\newcommand{\er}{R}

\newcommand{\norm}[1]{{\|{#1}\|}}

\newcommand{\mb}{\mathbb{B}}
\newcommand{\smb}{\mathbb{B}^{\circ}}
\newcommand{\seqset}[1]{{{#1}^\text{*}}}
\newcommand{\cseq}{\mathcal{S}}
\newcommand{\cpp}{\mathbb{PP}}
\newcommand{\ZZ}{\mathbb{Z}_K}
\newcommand{\NK}{\mathbb{N_K}}
\newcommand{\rwcs}{\upvarphi}

\newcommand{\seq}[1]{{#1}}
\newcommand{\id}[1]{{[#1]}}  % Iverson bracket notation 
\newcommand{\szm}{\operatorname{sim}}
\newcommand{\mct}{\Phi}
\newcommand{\cl}{y} % Class
\newcommand{\clv}{\by}
\newcommand{\siml}{y}
\newcommand{\trp}{\top}


\newcommand{\scI}{\mathcal{I}}
\newcommand{\scU}{\mathcal{U}}

\newcommand{\yh}{\ensuremath{\hat{y}}}
\newcommand{\one}{\ensuremath{\mathbf{1}}}
\newcommand{\wt}[2]{\ensuremath{w_{#2}^{(#1)}}}
\newcommand{\wtt}[2]{\ensuremath{\left(w_{#2}^{(#1)}\right)^\top}}
\newcommand{\opt}{\ensuremath{w^*}}
\newcommand{\Amat}[2]{\ensuremath{A_{#2}^{(#1)}}}
\newcommand{\Ainv}[2]{\ensuremath{\left(A_{#2}^{(#1)}\right)^{-1}}}
\renewcommand{\v}[2]{\ensuremath{v_{#2}^{(#1)}}}
\newcommand{\y}[2]{\ensuremath{y_{#2}^{(#1)}}}
\newcommand{\est}[2]{\ensuremath{u_{#2}^{(#1)}}}
\newcommand{\ytil}{\ensuremath{\tilde{y}}}
\newcommand{\E}{\ensuremath{\mathbb{E}}}
\newcommand{\mist}[2]{\ensuremath{M_{#2}^{(#1)}}}
\newcommand{\M}{\ensuremath{\mathcal{M}}}
\newcommand{\hs}{\ensuremath{\hat{s}}}
\newcommand{\hj}{\ensuremath{\widehat{j}}}
\newcommand{\bbw}{\ensuremath{\bar{\bw}}}
\newcommand{\bM}{\ensuremath{\bar{M}}}
\newcommand{\bbb}{\ensuremath{\bar{\bb}}}
\newcommand{\bT}{\ensuremath{\bar{T}}}
\newcommand{\boldeta}{\ensuremath{{\boldsymbol{\eta}}}}


\newcommand{\half}{\ensuremath{\frac{1}{2}}}
\newcommand{\wunproj}{\ensuremath{\tilde{w}}}
\newcommand{\Cd}{C_{\delta}}
\newcommand{\Cdx}[1]{C_{\delta,{#1}}}
\newcommand{\CdS}{C_{\delta/S}}
\newcommand{\Cdxxx}[1]{C_{\delta/3S,{#1}}}

\newcommand{\dataset}{{\cal D}}
\newcommand{\fracpartial}[2]{\frac{\partial #1}{\partial  #2}}
%\newenvironment{proofof}[1]{\par\noindent{\bf Proof of~\protect{#1}:}}{\hfill$\Box$\\}
\newcommand{\field}[1]{\mathbb{#1}}
\newcommand{\diag}[1]{\mbox{\sc diag}\!\left\{{#1}\right\}}
\newcommand{\wh}{\widehat}
\newcommand{\tr}{\mbox{\sc tr}}
\newcommand{\delete}{\mbox{\sc delete}}
\newcommand{\connected}{\mbox{\sc Is-connected}}
\newcommand{\ci}{\mbox{\sc ClusterIndices}}
\newcommand{\bsigma}{\boldsymbol{\sigma}}
\newcommand{\bb}{\boldsymbol{b}}
\newcommand{\by}{\boldsymbol{y}}
\newcommand{\bz}{\boldsymbol{z}}
\newcommand{\bx}{\boldsymbol{x}}
\newcommand{\ba}{\boldsymbol{a}}
\newcommand{\bw}{\boldsymbol{w}}
\newcommand{\bu}{\boldsymbol{u}}
\newcommand{\bq}{\boldsymbol{q}}
\newcommand{\bv}{\boldsymbol{v}}
\newcommand{\bp}{\boldsymbol{p}}
\newcommand{\be}{\boldsymbol{e}}
\newcommand{\bzero}{\boldsymbol{0}}
\newcommand{\bPhi}{\boldsymbol{\Phi}}
\newcommand{\bphi}{\boldsymbol{\phi}}
\newcommand{\R}{\field{R}}
\newcommand{\yhat}{\wh{y}}
\newcommand{\spin}{\{-1,+1\}}
\newcommand{\loss}{\ell}
\newcommand{\aod}{A_{\otimes}}
\newcommand{\scH}{\mathcal{H}}
\newcommand{\scK}{\mathcal{K}}
\newcommand{\scM}{\mathcal{M}}
\newcommand{\scO}{\mathcal{O}}
\newcommand{\morm}[1][\cdot]{\norm{#1}}
\newcommand{\defeq}{\stackrel{\rm def}{=}}
\newcommand{\sgn}{\mbox{\sc sgn}}
\newcommand{\var}{\textsc{var}}
\newcommand{\bubar}{\overline{\bu}}
\newcommand{\tbphi}{\widetilde{\bphi}}
\newcommand{\vct}{\mbox{\sc vec}}



\renewcommand{\tilde}{\widetilde}
\newcommand{\aL}{{\tilde L}}
\newcommand{\abL}{{\tilde {L^\otimes}}}

\newcommand{\bW}{\boldsymbol{W}}
\newcommand{\bX}{\boldsymbol{X}}
\newcommand{\bV}{\boldsymbol{V}}
\newcommand{\bU}{\boldsymbol{U}}

\renewcommand{\Pr}{\mathbb{P}}
\newcommand{\hDelta}{\hat{\Delta}}

\newcommand{\phat}{\wh{p}}
\newcommand{\muhat}{\wh{\mu}}
\newcommand{\Fhat}{\wh{F}}
\newcommand{\theset}[2]{\left\{ {#1}\,:\,{#2} \right\}}
\newcommand{\Ind}[1]{\field{I}_{\{{#1}\}}}
\newcommand{\hx}{\wh{x}}
\newcommand{\sX}{\tilde{X}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}

\renewcommand{\v}[2]{\ensuremath{\bv_{#2}^{(#1)}}}
\newcommand{\w}[2]{\ensuremath{\bw_{#2}^{(#1)}}}
\newcommand{\ignore}[1]{}


\DeclareMathOperator*{\argmax}{argmax} 
\DeclareMathOperator*{\argmin}{argmin}

\newcommand{\trace}{\tr}

\newcommand{\CB}{\mbox{\sc cb}}
\newcommand{\sCB}{\widetilde \CB}
\newcommand{\TCB}{\mbox{\sc tcb}}
\newcommand{\sTCB}{\widetilde \TCB}
\newcommand{\sbx}{\widetilde \bx}
\newcommand{\clip}{\mbox{\sc clip}}




\long\def\authornote#1{%
        \leavevmode\unskip\raisebox{5.5pt}{\rlap{$\scriptstyle\diamond$}}%
        \marginpar{\raggedright\hbadness=10000
        \def\baselinestretch{.8}\tiny
        \it #1\par}}

\newcommand{\MJH}[1]{\footnote{\color{red}MJH: #1}}



\newcommand{\WM}{lw-twma-94}
\newcommand{\shaimetric}{SSN04}
\newcommand{\trackingexpert}{HW98}



==> setting.tex <==

%\vspace{-0.07in}
\section{Learning Setting}\label{s:setting}
%
As in previous work in this literature (e.g., \cite{icml14,cgz13}), we assume that user behavior similarity is represented by an underlying (and unknown) clustering over the set of users.
Specifically, if we let $\scU = \{1,\ldots, n\}$ be the set of $n$ users, we assume $\scU$ can be partitioned
into a small number $m$ of clusters $U_1, U_2, \ldots, U_{m}$, where $m$ is expected to be much smaller than $n$.
The meaning of this clustering is that users belonging to the same cluster $U_j$ tend to have similar behavior, while
users lying in different clusters have significantly diverging behavior.
Both the partition $\{U_1, U_2, \ldots, U_{m}\}$ and the common user behavior within each cluster are {\em unknown}
to the learning system, and have to be inferred on the fly based on past user activity.

The above inference procedure has to be carried out within a sequential decision setting where the learning system (henceforth ``the learne'') has to continuously adapt to the newly received information provided by the users. To this effect, the learning process is divided into a discrete sequence of rounds:  in round $t=1,2,\dots$, the learner receives a user index $i_t \in \scU$ to serve content to. Notice that
the user to serve may change at every round, though the same user can recur many times. The sequence $\{i_t\}$ is exogenously determined by the way users interact with the system, and is not under our control. In practice, very high unbalancedness levels of user activity are often observed. Some users are very active, many others are (almost) idle or newly registered users, and their preferences are either extremely sporadic or even do not exist~\cite{recsys13}. Along with $i_t$, the system receives in round $t$ a set of feature vectors $C_{i_t} = \{\bx_{t,1}, \bx_{t,2},\ldots, \bx_{t,c_t}\} \subseteq \R^d$ representing the content which is currently available for recommendation to user $i_t$. The learner picks some ${\bar \bx_t} = \bx_{t,k_t} \in C_{i_t}$ to recommend to $i_t$, and then observes $i_t$'s feedback in the form of a numerical payoff $a_t \in \R$. In this scenario, the learner's goal is to maximize its total payoff\, $\sum_{t=1}^T a_t$\, over a given number $T$ of rounds. 
When the user feedback the learner observes is only the click/no-click behavior, the payoff $a_t$ can be naturally interpreted
as a binary feedback, so that the quantity
\[
\frac{\sum_{t=1}^T a_t}{T}
\]
becomes a click-through rate (CTR), where
$a_t = 1$ if the recommended item ${\bar \bx_t}$ was clicked by user $i_t$, and $a_t = 0$, otherwise. In our experiments (Section \ref{s:exp}), when the data at our disposal only provide the payoff associated with the item recommended
by the logged policy,
% ---this is the case when logs are in turn the outcome of a recommendation policy---
CTR is our measure of prediction accuracy. On the other hand, when the data come with payoffs for all possible items in $C_{i_t}$, then our measure of choice will be the cumulative {\em regret} of the learner,\footnote
{
In fact, for the sake of clarity, our plots will actually display {\em ratios} of cumulative regrets and {\em ratios} of CTRs ---see Section \ref{s:exp} for details.
}
defined as follows. Let $a_{t,k}$ be the payoff associated in the data at hand with item $\bx_{t,k} \in C_{i_t}$. Then the regret $r_t$ of the learner at time $t$ is the extent to which the payoff of the best choice in hindsight at user $i_t$ exceeds the payoff of the learner's choice, i.e.,
\[
r_t = \Bigl(\max_{k = 1, \ldots, c_t}\, a_{t,k} \Bigl) - a_{t,k_t}~,
\]
and the cumulative regret is simply
\[
\sum_{t=1}^T r_t~.
\]
Notice that the round-$t$ regret $r_t$ refers to the behavior of the learner when predicting preferences of user $i_t$, thus the cumulative regret takes into duly account the relative ``importance" of users, as quantified by their activity level. The same claim also holds when measuring performance through CTR.

